SMMF: Square-Matricized Momentum Factorization for Memory-Efficient Optimization

We propose SMMF (Square-Matricized Momentum Factorization), a memory-efficient optimizer that reduces the memory requirement of the widely used adaptive learning rate optimizers, such as Adam, by up to 96%. SMMF enables flexible and efficient factorization of an arbitrary rank (shape) of the first and second momentum tensors during optimization, based on the proposed square-matricization and one-time single matrix factorization. From this, it becomes effectively applicable to any rank (shape) of momentum tensors, i.e., bias, matrix, and any rank-d tensors, prevalent in various deep model architectures, such as CNNs (high rank) and Transformers (low rank), in contrast to existing memory-efficient optimizers that applies only to a particular (rank-2) momentum tensor, e.g., linear layers. We conduct a regret bound analysis of SMMF, which shows that it converges similarly to non-memory-efficient adaptive learning rate optimizers, such as AdamNC, providing a theoretical basis for its competitive optimization capability. In our experiment, SMMF takes up to 96% less memory compared to state-of-the-art memory efficient optimizers, e.g., Adafactor, CAME, and SM3, while achieving comparable model performance on various CNN and Transformer tasks.

==> equations/lamma_01.tex <==
% n + A/n이 convex임을 증명 where n>0
\begin{equation}
    tx_1+(1-t)x_1 + A / (tx_1+(1-t)x_2) \le tx_1+tA/(x_1) + (1-t)x_2 + (1-t)A/x_2 \\
    A / (tx_1+(1-t)x_2) \le tA/(x_1) + (1-t)A/x_2 \\
\end{equation}

==> equations/proof_of_squarematrixlization_01.tex <==
\begin{equation}
    \label{eq:proof_of_squarematrixlization_01}
    n + m = n + \dfrac{A}{n} \\
\end{equation}

==> sections/conclusion.tex <==
\section{Conclusion}
%We introduce \optim (Square-Matricized Momentum Factorization), a memory-efficient optimizer that decreases the memory requirement of adaptive learning rate optimization methods, e.g., Adam and Adafactor. Given arbitrary-rank momentum tensors, \optim reduces the optimization memory usage through the proposed square-matricization and matrix compression of the first and second momentums. The empirical evaluation shows that \optim reduces up to 96\% of optimization memory when compared to existing memory-efficient optimizers, i.e., Adafactor, SM3, and CAME, with competitive optimization performance on various models (i.e., CNNs and Transformers) and tasks (i.e., image classification, object detection, and NLP tasks over full-training, pre-training, and fine-tuning). Our analysis of regret bound proves that \optim converges in a convex function with a similar bound of \ideanote{AdamNC}.
We introduce \optim, a memory-efficient optimizer that decreases the memory requirement of adaptive learning rate optimization methods, e.g., Adam and Adafactor. Given arbitrary-rank momentum tensors, \optim reduces the optimization memory usage through the proposed square-matricization and matrix compression of the first and second momentums. The empirical evaluation shows that \optim reduces up to 96\% of optimization memory when compared to existing memory-efficient optimizers, i.e., Adafactor, SM3, and CAME, with competitive optimization performance on various models (i.e., CNNs and Transformers) and tasks (i.e., image classification, object detection, and NLP tasks over full-training, pre-training, and fine-tuning). Our analysis of regret bound proves that \optim converges in a convex function with a similar bound of \ideanote{AdamNC}.

==> sections/convergence.tex <==
\section{Regret Bound Analysis}
\label{sec:regret}
We analyze the convergence of \optim by deriving the upper bound of the regret that indicates an optimizer's convergence~\cite{adam}. The regret $R(T)$ is defined as the sum of differences between two convex functions $f_t(\weight_t)$ and $f_t(\weight^*)$ for all $t \in [1, T]$, where $\VECTOR{w}^*$ is an optimal point.
\ninefont
\begin{equation}
    \label{eq:regret}
    R(T) = \sum_{t = 1}^T(f_t(\VECTOR{w}_t) - f_t(\VECTOR{w}^*))
\end{equation}
\tenfont
Since \optim factorizes (compresses) the momentum tensors, unlike Adam, we introduce some compression error terms in our analysis as follows. First, $\hat{\VECTOR{m}}_t$ and $\hat{\VECTOR{v}}_t$ are the decompressed and vectorized vectors of the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum $\MATRIX{M}_t$ and $\MATRIX{V}_t$, containing $\VECTOR{e}_{m, t}$ and $\VECTOR{e}_{v, t}$, which denote compression errors of $\MATRIX{M}_t$ and $\MATRIX{V}_t$, respectively, i.e., $\VECTOR{e}_{m, t} = \hat{\VECTOR{m}}_t - \VECTOR{m}_t$ and $\VECTOR{e}_{v, t} = \hat{\VECTOR{v}}_t - \VECTOR{v}_t$. Similarly, we also define $\tilde{\VECTOR{e}}_{m, t}$, $\tilde{\VECTOR{e}}_{v, t}$, $\tilde{\VECTOR{g}}_{m, t}$, $\tilde{\VECTOR{g}}_{v, t}$, and $\hat{\VECTOR{g}}_{m, t}$. The detailed definitions are given in \Cref{lemma:compact_form_of_m_and_v_hat,lemma:m_t_with_g_tilde} in \Cref{proof:regret_bounding}.
\begin{theorem}
    \label{thm:regret_bounding}
    Let $\weight_t$ and $\VECTOR{v}_t$ be the vectorized $\WEIGHT_t$ and $\MATRIX{V}_t$, respectively, in \Cref{alg:brief_algorithm}, and $\eta_t = \eta / \sqrt{t}$, $\beta_1 = \beta_{1, 1}$, $\beta_2 = \beta_{2, 1}$, $\beta_{1, t} \leq \beta_1$ for all $t \in [1, T]$, and $\zeta_1 > 0$. We assume that $\lvert\lvert \weight_t - \weight^*\rvert\rvert_2 \leq D$, $\lvert\lvert \weight_k - \weight_l\rvert\rvert_{\infty} \leq D_{\infty}$, and all $\weight$ is in $\mathcal{F}$ where $D$ is the diameter of the feasible space $\mathcal{F}$. Furthermore, let $\beta_{1, t}$ and $\beta_{2, t}$ follow the following conditions, where the conditions (a) and (b) are from \cite{amsgrad}.
    \ninefont
    \begin{align*}
        \label{cond:01}
        & (a) ~\eta_{t - 1}\sqrt{\VECTOR{v}_{t, i}} \geq \eta_{t} \sqrt{\VECTOR{v}_{t - 1, i}} \\
        & (b) ~\dfrac{1}{\eta_t} \sqrt{\sum_{j = 1}^t \prod_{k = 1}^{t - j} \beta_{2, t - k + 1}(1 - \beta_{2, j} \tilde{\VECTOR{g}}_{v, j, i})} \geq \dfrac{1}{\zeta_2} \sqrt{\sum_{j = 1}^t \tilde{\VECTOR{g}}_{v, j, i}} \\ 
        & \quad\,for\,some\,\zeta_2 > 0\,and\,all\,t \in [:T]
    \end{align*}
    \tenfont
    Given the above conditions, the upper bound of the regret $R(T)$ on a convex function becomes:
    \ninefont
    \begin{align}
        R(T)
            &\leq \sum_{i = 1}^d \dfrac{D^2 \sqrt{\VECTOR{v}_{T, i}}}{2\eta_T (1 - \beta_1)}  + \sum_{t = 1}^T \sum_{i = 1}^d\dfrac{\beta_{1, t} D_{\infty}^2 \sqrt{\VECTOR{v}_{t, i}}}{2 \eta_{t} (1 - \beta_{1, t})} \\
            \nonumber
            & \quad +\dfrac{\zeta_1 \zeta_2 (1 + \beta_1) \sqrt{d}}{(1 - \beta_1)^3} \sqrt{\sum_{i = 1}^d \lvert \lvert \VECTOR{g}_{1:T, i} \rvert \rvert_2} ~ .
    \end{align}
    \tenfont
\end{theorem}
The full proof of \Cref{thm:regret_bounding} is provided in \Cref{proof:regret_bounding}. It shows that \optim has a similar regret bound ratio to AdamNC~\cite{amsgrad} (a variant of Adam), i.e., $\BIGO{\sqrt{T}}$ where $T$ is the total optimization steps, under the conditions (a) and (b). It allows \optim to perform consistent optimization comparable to Adam-based and existing memory-efficient optimizers, as shown in the experiment (\Cref{sec:experiment}). The conditions (a) and (b) can be satisfied \ideanote{by properly scheduling $\beta_{2, t}$~\cite{amsgrad}}.

==> sections/experiment.tex <==
\section{Experiment}
\label{sec:experiment}
We implement the proposed \optim using PyTorch~\cite{pytorch}, which is available both on an GitHub and in \Cref{sec:code}. For evaluation, we compare the memory usage and optimization performance of \optim against four (memory-efficient) optimizers, i.e., Adam, Adafactor, SM3, and CAME, with two types of deep learning tasks: 1) CNN models for image tasks and 2) Transformer models for NLP tasks. \ideanote{The detailed experimental setups and training configurations are provided in \Cref{config:training_configurations}.}

\noindent\textbf{CNN-based Models and Tasks.} We apply the five optimizers, including \optim, to two representative image tasks, i.e., image classification and object detection, and evaluate them by 1) training ResNet-50~\cite{resnet} and MobileNetV2~\cite{mobilenet} on CIFAR100~\cite{cifar} and ImageNet~\cite{imagenet}, and 2) training YOLOv5s and YOLOv5m~\cite{ultralytics2021yolov5} on COCO~\cite{lin2015microsoft}.

\noindent\textbf{Transformer-based Models and Tasks.} For NLP tasks, we train several Transformer-based models  \ideanote{from small scale to large scale} with three training methods, i.e., full-training, pre-training, and fine-tuning. We 1) full-train Transformer-base and big models~\cite{transformer} on WMT32k~\cite{bojar2014findings_wmt32k}, 2) pre-train BERT~\cite{bert}, GPT-2~\cite{gpt2}, and T5~\cite{t5} on BookCorpus~\cite{bookcorpus} \& Wikipedia, and 3) fine-tune BERT, GPT-2, T5-small, and LLaMA-7b~\cite{llama1} on QNLI, MNLI, QQP, STSB, and MRPC~\cite{glue} datasets. To fine-tune LLaMA-7b, we use LoRA~\cite{lora}. Additionally, we train various Transformer models on other NLP tasks such as question-answering~\cite{squad,squadv2}, translation~\cite{wmt16}, and summarization~\cite{cnn_dailymail,xsum,ilpost}.  Due to the page limit, we provide the detailed experiment results in \Cref{sec:additional_fine_tuning_performance}.

\noindent\textbf{Optimization Time Measurement.} We measure the optimization time of five optimizers with the CNN and Transformer models, i.e., 1) MobileNetV2 and ResNet-50 on ImageNet, 2) Transformer-base and big on WMT32K.
\input{tables/memory_footprint_and_result_of_cnn_models}
\subsection{CNN-based Models and Tasks}
\label{subsec:cnn_models_training}

\textbf{Image Classification.} The first and second tables of \Cref{tab:memory_footprint_and_result_of_cnn_models} summarize the optimizer memory usage, end-to-end training (one-batch) memory usage, and top-1 classification accuracy of MobileNetV2 and ResNet-50 on CIFAR100 and ImageNet, respectively, showing that \optim achieves comparable accuracy among the five optimizers with the lowest memory footprint. For instance, for ResNet-50 on ImageNet, \optim substantially reduces the optimizer memory usage from 220 to 3.7 MiB (59x smaller) compared to Adafactor while achieving a higher accuracy (73.7\%). Its memory usage is also smaller than the other two memory-efficient optimizers, i.e., SM3 (99 vs. 3.7 MiB) and CAME (346 vs. 3.7 MiB). On the other hand, both Adafactor and CAME take more memory than not only \optim but also Adam due to the overhead of slicing the momentum tensor into multiple matrices for factorization based on the last two rank of the tensor corresponding to the size of a CNN kernel (i.e., $C^i_k\times C^o_k \times H_k \times W_k$). Since $H_k$ and $W_k$ are usually small, e.g., $H_k=W_k=1$, $3$ or $5$, whereas $C^i_k$ and $C^o_k$ are large, e.g., $512$, the memory reduction effect of both Adafactor and CAME becomes marginal in CNNs. \Cref{fig:cnn} (left) plots the top-1 validation accuracy of MobileNetV2 on ImageNet over training steps. 

\input{images/cnn_model_performance}
\noindent\textbf{Object Detection.} The third table of \Cref{tab:memory_footprint_and_result_of_cnn_models} summarizes the optimizer memory usage, end-to-end training (one-batch) memory usage, and the model performance metric (i.e., mAP50) of YOLOv5s and YOLOv5m on the COCO object detection task. \Cref{fig:cnn} (right) shows the mAP50 of YOLOv5s on COCO over training steps. Similar to image classification tasks, \optim achieves comparable mAP50, e.g., 59.6 in YOLOv5m and 54.1 in YOLOv5s, over all the four optimizers with the lowest memory up to 78x reduction, e.g., 267 vs. 3.4 MiB. This result implies that YOLOv5s (65 MiB) can be trained on an off-the-shelf memory-constrained device, e.g., Coral Dev Micro (64 MiB)~\cite{coral_devboard_micro}, along with other memory-efficient training methods such as gradient checkpointing~\cite{gradient_checkpointing}.

These experiment results show that \optim performs consistent and reliable optimization for both image classification and object detection tasks with different CNN models, taking the smallest memory compared to existing memory-efficient optimizers, i.e., Adafactor, SM3, and CAME. % while taking
\input{tables/memory_footprint_and_result_of_full_training}

\subsection{Transformer-based Models and Tasks}
\label{subsec:transformer_models_training}
\textbf{Full-training.} As shown in \Cref{tab:memory_footprint_and_result_of_full_training}, \optim achieves comparable perplexity with up to 70x smaller optimizer memory when full-training (i.e., training models from scratch) both the Transformer-base and big models. Since \optim square-matricizes both the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentums and factorizes them, its memory usage is at least half lower than the other memory-efficient optimizers, i.e., Adafactor, SM3, and CAME. Given that most Transformer architectures consist of two-dimensional matrices, e.g., attention and linear layers, the memory reduction effect of SM3 that is good at compressing a high-rank tensor, becomes insignificant, making its memory usage similar to Adafactor and CAME. On the other hand, \optim can effectively reduce memory required to factorize a two-dimensional matrix with square-matricization, e.g., saving 69\% of memory for the embedding weight matrix of BERT, as the weight matrix in $\RSET^{30522\times768}$ becomes $\RSET^{5087\times4608}$. Although the square-matricization may spoil the gradient pattern of the Transformer's weight parameters~\cite{sm3}, \optim performs comparable optimization (e.g., 6.7 perplexity for WMT32k) using much less memory by fully utilizing the intact latest gradient before it is compressed. It is possible by taking the proposed $decompression$$\rightarrow$$compression$ scheme that first reflects the intact gradient pattern, if any, to the momentum and then performs factorization, unlike existing optimizers, e.g., Adafactor, SM3, and CAME, which apply the $compression$$\rightarrow$$decompression$ scheme. \Cref{fig:transformer_base_ppl} (left) shows the test perplexity of the Transformer-base model full-trained on WMT32k from scratch.

\input{tables/memory_footprint_and_result_of_pre_training}

\noindent\textbf{Pre-training.} \Cref{tab:memory_footprint_and_result_of_pre_training} shows the optimizer memory usage including $\MATRIX{S}_{\MATRIX{M}}$, end-to-end training (one-batch) memory usage, and the perplexity of BERT, GPT-2, and T5 pre-trained for the BookCorpus \& Wikipedia dataset. For GPT-2 pre-trained with Adafactor, we failed to obtain its perplexity since it diverged (NaN) even with multiple trials of various settings, e.g., different machines, hyper parameters, seeds, etc. On the other hand, \optim performs competitive optimization for all pre-training of BERT, GPT-2, and T5 using up to 60x lower optimizer memory. \Cref{fig:transformer_base_ppl} (right) shows that \optim (yellow) curtails the optimizer memory usage in the pre-training of BERT about 1.26 GiB (from 1.3 to 0.04 GiB) while exhibiting the similar test perplexity trajectory to CAME (purple) taking much more memory to maintain the similar optimization performance. Overall, Adafactor, CAME, and \optim show similar perplexity trajectories, confirming that \optim retains the optimization performance in pre-training of Transformers with the lowest memory, enabled by 1) square-matricization of any rank (shape) of momentums (e.g., a vector, matrix, tensor, etc.) and 2) the $decompression$$\rightarrow$$compression$ scheme that uses the uncompressed gradients at the current update step. They jointly allow it to pre-train Transformers aptly during a massive number of pre-training steps by persistently conducting effective and efficient optimization over a long time horizon.

That being said, \optim also exhibits some occasional loss spike~\cite{loss-spike-01, loss-spike-02} at the early steps of optimization (training), which stabilizes as the training proceeds. It is a well-known phenomenon that commonly occurs in the pre-training of many large language models~\cite{t5, gpt2} optimized with existing optimizers, such as Adam, Adafactor, SM3, and CAME. We discuss it in more detail in \Cref{sec:limitation}.

\noindent\textbf{Fine-tuning.} \Cref{tab:memory_footprint_and_result_of_fine_tuning} summarizes the optimization memory usage including $\MATRIX{S}_{\MATRIX{M}}$, end-to-end training(one-batch) memory usage, and the model performance of GPT-2, T5-small, and LLaMA-7b, which are fine-tuned for the QNLI, MNLI, QQP, STSB, and MRPC datasets from pre-trained models. As shown in the table, \optim achieves comparable model performance in the six datasets compared to the other four optimizers with the lowest memory usage. For instance, \optim provides similar accuracy (90.6\%) for GPT-2 on QQP compared to CAME, using much smaller optimizer and end-to-end training memory, respectively (16 vs. 489 MiB and 0.96 vs. 1.43 GiB). It demonstrates that \optim is also apt at fine-tuning Transformer models, which entails delicate and intricate updates of weight parameters, otherwise likely to degrade the learning performance for downstream tasks. In practice, it suggests that some Transformer models, such as T5, would be fine-tuned on a low-end device, e.g., \ideanote{Raspberry Pi Zero (0.5 GiB)}, with similar model performance to CAME (i.e., 83.0\% vs. 82.8\%), as \optim curtails the end-to-end training memory requirement of fine-tuning down to 0.47 GiB. On the other way around, \optim can scale up training of Transformers by enabling memory-efficient optimization of enormous Transformer models that require a gigantic amount of memory, e.g., \ideanote{hundreds} of GiB. 

Similar to the CNN-based models and tasks, the experimental results of Transformers demonstrate that \optim steadily performs competitive optimization for a wide range of Transformer models, tasks, and training methods (i.e., full-, pre-, and fine-tuning) with the smallest memory usage.

\input{tables/memory_footprint_and_result_of_fine_tuning}
\input{tables/time}
\input{images/transformer_base_ppl}
\subsection{Optimization Time Measurement}
\label{subsec:optimization_time}
\Cref{tab:time} shows the optimization time measured for a single training step of the five optimizers when training MobileNetV2 and ResNet-50 on ImageNet, and Transformer-base and big on WMT32k. Except for Adam, the four optimizers take similar optimization times, where \optim takes a little more time than the other three. That is because it trades off the memory space and optimization time, i.e., the time required for square-matricization and the sign matrix operations for the \ideanote{$1^{st}$} momentum (\Cref{alg:matrix_decompression,alg:matrix_compression}). However, \optim offers huge memory reduction compared to the amount of the increased optimization time, e.g., \ideanote{7.9x} memory reduction vs. 1.2x time increase for Adam and \optim with the 8-bit format $\boldsymbol{S_{M}}$ in \Cref{alg:matrix_decompression,alg:matrix_compression} applied to Transformer-big on WMT32k, and \ideanote{7.8x} vs. 1.6x for Adam and \optim with  $\boldsymbol{S_{M}}$ applied to ResNet-50 on ImageNet.

==> sections/limitation.tex <==
\section{Limitations and Discussions}
\label{sec:limitation}

\textbf{Overhead of Binary Signs.} 
It is not easy to effectively factorize the \ideanote{$1^{st}$} momentum $\MATRIX{M}$ having negative elements. While \optim circumvents this by storing the binary sign matrix (1-bit) that is much smaller than the original matrix (32-bit), there are some methods that can further reduce the memory required to store the sign matrix. For instance, Binary Matrix Factorization \cite{bmf2,bmf3} can be employed to factorize the binary matrix into two lower-rank matrices, reducing the memory space for storing the binary matrix with a high restoration rate.

\noindent\textbf{Optimization Time.} \Cref{sec:comput_complexity} finds that the time complexity of \optim is similar to existing memory-efficient optimizers, e.g., \ideanote{Adafactor}, showing that \optim effectively saves a significant amount of memory (up to 96\%) compared to them with slightly increased optimization time.

\noindent\textbf{Loss Spike at Initial Training Steps.} We observe some loss spike at the initial training steps, especially in Transformer models, which is a well-known issue commonly observed in other works~\cite{loss-spike-01,loss-spike-02} and many optimizers, i.e., Adam (with the bias correction term), Adafactor, SM3, and CAME. With appropriate hyper-parameter tuning, e.g., learning rate and \ideanote{weight-decay}, it can be stabilized as the training proceeds, like other optimizers.

\noindent\textbf{Extremely Large Models and Other Tasks.} 
Due to the limited computing resources, we have not been able to experiment \optim with extremely large models, e.g, GPT-4~\cite{gpt4}, LLaMA-2 70B~\cite{llama2}, and diffusion models~\cite{ldm}. From our theoretical study and empirical result, we expect \optim to perform competitive optimization with them. We hope to have a chance to test \optim with them.

==> sections/ours.tex <==
\section{\optim \\ (Square-Matricized Momentum Factorization)}
\label{sec:smmf}
\input{algorithms/brief_algorithm}
\Cref{alg:brief_algorithm} shows the overall procedure of the proposed \optim (Square-Matricized Momentum Factorization), applied to the weight tensor (momentum) at each layer of the model. In short, given the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum tensors as $\MATRIX{M}, \MATRIX{V} \in \RSET^{n_1 \times \ldots \times n_d}$, \optim reduces the memory complexity required for optimization into $\BIGOU{M}{\hat{n} + \hat{m}}$ and $\BIGOU{V}{\hat{n} + \hat{m}}$ for $\MATRIX{M}$ and $\MATRIX{V}$, respectively, with $\hat{n},\hat{m}=\arg\min_{n, m}\lvert n - m \rvert$ such that $n m = \prod_{r=1}^{d}n_r$ where $n_r, n, m, \hat{n}$, and $\hat{m}$ are in $\NSET$. It first transforms $\MATRIX{M}, \MATRIX{V} \in \RSET^{n_1 \times \ldots \times n_d}$ into a matrix closest to the square (square-matricization), i.e., $\MATRIX{M}, \MATRIX{V} \in \RSET^{\hat{n} \times \hat{m}}$ where $\hat{n} \simeq \hat{m}$, and then applies \ideanote{NNMF} (\Cref{alg:nnmf}) to $\MATRIX{M}, \MATRIX{V} \in \RSET^{\hat{n} \times \hat{m}}$ \ideanote{as one-time} single matrix factorization (compression). Since the \ideanote{$1^{st}$} momentum $\MATRIX{M}$ can be negative, unlike the \ideanote{$2^{nd}$} momentum $\MATRIX{V}$ that is non-negative, we apply NNMF to the absolute values of $\MATRIX{M}$ and store the sign of each element of $\MATRIX{M}$ as a separate set of binary values (1-bit). Although it incurs extra memory overhead $\BIGOU{M}{\hat{n} \hat{m}}$ on top of $\BIGOU{M}{\hat{n} + \hat{m}}$ and $\BIGOU{V}{\hat{n} + \hat{m}}$, its memory footprint is 32 times smaller than storing the original $\MATRIX{M}$ with the 32-bit floating-point format. The following subsections describe each step of \optim.
\input{algorithms/square_matrixlization}
\subsection{Square-Matricization}
\label{sec:square-matricization}
In \Cref{alg:brief_algorithm}, \optim first obtains a rank-$d$ gradient $\MATRIX{G}_t \in \RSET^{n_1\times \ldots \times n_d}$ for the weight and bias tensor at each layer of the model and converts it into a matrix closest to a square matrix $\bar{\MATRIX{G}}_t \in \RSET^{\hat{n} \times \hat{m}}$ where $\hat{n} \simeq \hat{m}$, for factorization, naturally leading to the square-matricization of the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum, $\MATRIX{M}$ and $\MATRIX{V}$. To this end, we propose a square-matricization method that reshapes $\MATRIX{G}_{t} \in \RSET^{n_1 \times \ldots \times n_d}$ into a matrix closest to a square matrix $\bar{\MATRIX{G}}_{t} \in \RSET^{\hat{n} \times \hat{m}}$ such that $n m = \prod_{r=1}^{d} n_{r}$ and $(\hat{n}, \hat{m}) = \arg\min_{n, m}(n + m) = \arg\min_{n, m}\lvert n - m \rvert$, where $\hat{n}, \hat{m}, n, m \in \NSET$. Following theorems show that the square-matricization of $\bar{\MATRIX{G}}_t \in \RSET^{\hat{n} \times \hat{m}}$, i.e., having $\hat{n} \simeq \hat{m}$, also minimizes $\hat{n} + \hat{m}$.

\begin{theorem}    \label{thm:the_theorem_of_square_matrixlization_discrete2}    
    Given $n_r \in \NSET$, $r \in [1, d]$, and a constant $\SCALAR{N} = \prod_{r=1}^d n_r$, then $\prod_{r=1}^{d-2} n_r(n_{d-1} + n_d)$ decreases if both $n_{d-1}$ and $n_d$ increase (Proof provided in \Cref{proof:the_theorem_of_square_matrixlization_discrete2}).
\end{theorem}
\begin{corollary}
    \label{cor:the_theorem_of_square_matrixlization_discrete2}
    Given $\SCALAR{N} = \prod_{r=1}^d n_r$, there exist $N = \hat{n} \hat{m}$ such that $\hat{n} + \hat{m} = \min \prod_{r=1}^{d-2} n_r(n_{d-1} + n_d)$, $(\hat{n}, \hat{m}) \in \NSET$. % where $\hat{n}, \hat{m} \in \NSET$
\end{corollary}
\begin{theorem}
    \label{thm:the_theorem_of_square_matrixlization_discrete}
    Given $n_r, n, m \in \NSET$, $r \in [1, d]$, $\SCALAR{N} = \prod_{r=1}^d n_r = nm$, and $n \leq m$, then $\hat{n}, \hat{m} = \arg\min_{n, m}(n + m) = \arg\min_{n, m}\lvert n - m \rvert$ (Proof provided in \Cref{proof:the_proof_of_square_matrixlization_discrete}).
\end{theorem}
From \Cref{cor:the_theorem_of_square_matrixlization_discrete2}, square-matricizing $\MATRIX{G}_t \in \RSET^{n_1 \times \ldots \times n_d}$ into $\bar{\MATRIX{G}}_t \in \RSET^{\hat{n} \times \hat{m}}$ reduces the memory complexity since $\prod_{r=1}^{d-2} n_r(n_{d-1} + n_d) \leq \prod_{r=1}^d n_r$. Also, based on \Cref{thm:the_theorem_of_square_matrixlization_discrete}, minimizing $\lvert n - m \rvert$ is equivalent to minimizing $n + m$. From this, we derive the square-matricization algorithm (\Cref{alg:square_matrixlization}) that finds $\hat{n}$ and $\hat{m}$, which minimizes $\hat{n}+\hat{m}$ by solving $(\hat{n}, \hat{m}) = \arg\min_{n, m} \lvert n - m \rvert$. By reshaping a rank-$d$ gradient into a matrix closest to a square matrix through square-matricization, it becomes able to perform one-time single matrix factorization, which minimizes the memory complexity of $\BIGOU{M, V}{\hat{n} + \hat{m}}$ for the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum $\MATRIX{M}$ and $\MATRIX{V}$. Thus, the memory usage of \optim becomes smaller than those of existing memory-efficient optimizers~\cite{adafactor, came} that should slice a high-rank tensor into a bunch of matrices for multiple factorizations, i.e., $\BIGO{\prod_{r = 1}^{d - 2} n_r (n_{d - 1} + n_d)}$ given $\MATRIX{V} \in \RSET^{n_1 \times \ldots \times n_d}$. That is, the memory complexity of CNNs having high-rank gradient tensors grows over the rank of gradients~\cite{adafactor, came}, whereas that of \optim does not.

\subsection{Decompression and Compression}
\label{sec:decompression_and_compression}
\textbf{Decompression $\rightarrow$ Compression.} After square-matricizing the gradient, \optim decompresses the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum from two vectors factorized at the previous step $t{-}1$ to update the momentums, as in \Cref{alg:brief_algorithm}. Then, it compresses the momentums obtained at step $t$ into vectors and updates the weight $\WEIGHT$ using the decompressed momentums. We call this process the $decompression \rightarrow compression$ scheme, in which the gradient $\bar{\MATRIX{G}}_t$ at the current step $t$ is reflected to the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum before it is factorized, enabling the precise update of the weight.

The significance of information in the current gradient, e.g., tensor patterns, has been emphasized in some previous works~\cite{sm3}. Since reshaping and factorization of the gradient may ruin some potentially important patterns of the momentums contained in the previous gradient $\MATRIX{G}_{\tau < t}$, reflecting the current gradient $\MATRIX{G}_t$ (and its pattern) is crucial in model performance. Thus, by performing decompression with $\MATRIX{G}_t$ prior to updating and compressing (factorizing) $\MATRIX{M}_t$ and $\MATRIX{V}_t$, it is expected to improve the optimization performance. On the contrary, existing optimizers, such as Adafactor, first compress  $\MATRIX{G}_t$ and then updates momentums through decompression, which we call the $compression \rightarrow decompression$ scheme. In this scheme, some useful information of $\MATRIX{G}_t$ would be lost by compression (factorization), implying that an optimizer can hardly utilize the intact state of $\MATRIX{G}_t$, likely to degrade the model performance.
\input{algorithms/matrix_decompression}
\noindent\textbf{Decompression.} First, in the decompression phase (\Cref{alg:matrix_decompression}), the \ideanote{$1^{st}$} and \ideanote{$2^{nd}$} momentum, \{$\hat{\lvert \MATRIX{M}}_{t-1} \rvert$, $\hat{\MATRIX{V}}_{t-1}$\} $\in \RSET^{\hat{n} \times \hat{m}}$, are defactorized from the two vectors for each, i.e., \{$\VECTOR{r}_{\MATRIX{M}_{t-1}}, \VECTOR{c}_{\MATRIX{M}_{t-1}}$\} for $\lvert \hat{\MATRIX{M}}_{t-1} \rvert$ and $\{\VECTOR{r}_{\MATRIX{V}_{t-1}}$, $\VECTOR{c}_{\MATRIX{V}_{t-1}}\}$ for $\hat{\MATRIX{V}}_{t-1}$, which have been factorized from the square-matricized momentums at the previous step $t$$-$$1$, by performing outer product between them. To apply NNMF to the \ideanote{$1^{st}$} momentum $\boldsymbol{\hat{M}}_{t}$, its sign values are stored as a binary matrix $\MATRIX{S}_{\MATRIX{M}_{t-1}}$$\in$$ \BSET^{\hat{n} \times \hat{m}}$ in the compression phase and restored back to the defactorized \ideanote{$1^{st}$} momentum $\boldsymbol{\hat{M}}_{t}$ in an element-wise manner. Then, $\boldsymbol{M}_{t}$ and $\boldsymbol{V}_{t}$ are updated by using two coefficients $\beta_{1, t}$ and $\beta_{2, t}$.

\input{algorithms/matrix_compression}
\noindent\textbf{Compression.} Next, in the compression phase (\Cref{alg:matrix_compression}), the sign values of $\MATRIX{M}_t$ is stored as a binary sign matrix $\MATRIX{S}_{\MATRIX{M}_t}$ for the next step of optimization, and both $\lvert \MATRIX{M}_t \rvert$ and $\MATRIX{V}_t$ are factorized into two vectors for each, i.e., $\{ \boldsymbol{r}_{M_{t}},\boldsymbol{c}_{M_{t}} \}$ and $\{ \boldsymbol{r}_{V_{t}},\boldsymbol{c}_{V_{t}} \}$, respectively. To reduce the computation required for compression, it determines whether to normalize $\VECTOR{r}$ or $\VECTOR{c}$ based on the shape of the matrix.

\noindent\textbf{Weight Update.} Lastly, the weight update term $\boldsymbol{U}\in \mathbb{R}^{\hat{n}\times\hat{m}}$ is computed as  $\boldsymbol{M}_{t}/\sqrt{\boldsymbol{V}_{t}+\epsilon}$ and reshaped back into the original dimension of the gradient $\boldsymbol{G}_{t} \in \mathbb{R}^{n_1\times \ldots \times n_d}$ to update the weight $\boldsymbol{W}_{t}$.

\subsection{Time (Computation) Complexity of \optim} 
\label{sec:comput_complexity}
The time complexity of SMMF consists of two parts, i.e., square-matricization and decompression/compression. First, computing $\hat{n}$ and $\hat{m}$ for square-matricization (\Cref{alg:square_matrixlization}) is $\BIGO{\sqrt{N}}$, where $N$ is the number of elements in the momentum tensor. However, this computational overhead is negligible since $\hat{n}$ and $\hat{m}$ are calculated only once before starting model training (optimization). Next, the time complexity of decompression (\Cref{alg:matrix_decompression}) and compression (\Cref{alg:matrix_compression}) are both $\BIGO{N}$, which is asymptotically equivalent to existing memory-efficient optimizers, i.e., Adafactor and CAME. While taking a similar computational complexity to existing memory-efficient optimizers~\cite{adafactor,came}, \optim is able to save up to 96\% of memory, as shown in \Cref{sec:experiment}.

==> tables/configs_transformer_dataset03.tex <==
\begin{table*}[hbt!]
\caption{The pre-training BERT. GPT2 and T5 configurations using Adam, Adafactor, SM3, CAME and {\optimizername} on dataset03. $\lambda$ means the growth-rate for first momentum, $\gamma$ means the decay-rate for second momentum, $d$ means the clip-threshold, and x means the configuration is not for the optimizer.}
\label{tab:configs_transformer_dataset03}
\begin{center}
    \begin{small}
        \begin{tabular}{l|c|c|c|c|c|c}
        \toprule
        \multicolumn{7}{c}{Pre-training Configurations on ???} \\
        
        \midrule
        \multicolumn{1}{l|}{Model} & Configurations & Adam & Adafactor & SM3 & CAME &{\optimizername} \\

        \bottomrule
        BERT & epochs & 1 & 1 & 1 & 1 & 1 \\
         & batch size & 1 & 1 & 1 & 1 & 1 \\
         & learning-rate & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_2$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_3$ & x & x & x & 1 & x \\
         & $\gamma$  & x & -0.8 & x & 1 & 1 \\
         & $d$ & x & 1 & x & 1 & x \\
         & $\lambda$ & x & x & x & x & 1 \\
         & $\epsilon_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\epsilon_2$ & 1 & 1 & 1 & 1 & 1 \\
        \hline
        
        GPT2 & epochs & 1 & 1 & 1 & 1 & 1 \\
         & batch size & 1 & 1 & 1 & 1 & 1 \\
         & learning-rate & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_2$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_3$ & x & x & x & 1 & x \\
         & $\gamma$  & x & -0.8 & x & 1 & 1 \\
         & $d$ & x & 1 & x & 1 & x \\
         & $\lambda$ & x & x & x & x & 1 \\
         & $\epsilon_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\epsilon_2$ & 1 & 1 & 1 & 1 & 1 \\
        \hline
        
        T5 & epochs & 1 & 1 & 1 & 1 & 1 \\
         & batch size & 1 & 1 & 1 & 1 & 1 \\
         & learning-rate & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_2$ & 1 & 1 & 1 & 1 & 1 \\
         & $\beta_3$ & x & x & x & 1 & x \\
         & $\gamma$  & x & -0.8 & x & 1 & 1 \\
         & $d$ & x & 1 & x & 1 & x \\
         & $\lambda$ & x & x & x & x & 1 \\
         & $\epsilon_1$ & 1 & 1 & 1 & 1 & 1 \\
         & $\epsilon_2$ & 1 & 1 & 1 & 1 & 1 \\
        \hline
        \end{tabular}
    \end{small}    
\end{center}
\end{table*}

==> tables/memory_footprint_reduction_cnn_transformer.tex <==
\begin{table}[hbt!]
\setlength\tabcolsep{2pt}
\captionsetup{font=small}
\caption{Memory usage reduction of ResNet-50 and Transformer-base respectively trained on CIFAR100 and WMT32k using Non-SquareMatricization and Square-Matricization without first momentum. The Non-Square-Matricization method is identical to Adafactor.}
\label{tab:memory_footprint_reduction_cnn_transformer}
\begin{center}
    \begin{footnotesize }
        \begin{tabular}{l|c|c}
        \toprule
        \multicolumn{3}{c}{Optimizer Memory [MiB] (Reduction Percentage \%)} \\
        \midrule
        Method & ResNet-50 &  Transformer-base\\
        \bottomrule
        \textbf{Square-Matricization} & \textbf{0.33} (\textbf{0.26\%}) & \textbf{1.5} (\textbf{50\%})\\
        Non-Square-Matricization & 125 (100\%) & 3 (100\%)\\
        \end{tabular}
    \end{footnotesize }    
\end{center}
\end{table}

==> tables/scheduling.tex <==
\begin{table}[hbt!]
\caption{The effect of $\beta_1$ and $\beta_2$ scheduling using ResNet50 on CIFAR100. $\gamma$ means the decay-rate for second momentum and $\lambda$ means growth-rate for first momentum.} \label{tab:scheduling}
\begin{center}
    \begin{small}
        \begin{tabular}{c|c|c}
        \toprule
        \multicolumn{3}{c}{Training Accuracy over Various Scheduling Configurations} \\
        \midrule
        $\gamma$ & $\lambda$ & ACC (\%)\\
        \bottomrule
        -0.8 & 0.999 & ??.?\% \\ 
        -0.5 & 0.999 & ??.?\% \\ 
        -0.8 & 0.99 & ??.?\% \\ 
        -0.5 & 0.99 & ??.?\% \\ 
        -0.8 & 0.9 & ??.?\% \\ 
        -0.5 & 0.9 & ??.?\% \\ 
        \end{tabular}
    \end{small}    
\end{center}
\end{table}
